Speeding up Heterogeneous Federated Learning with Sequentially Trained Superclients

Federated Learning (FL) allows training machine learning models in privacy-constrained scenarios by enabling the cooperation of edge devices without requiring local data sharing. This approach raises several challenges due to the different statistical distribution of the local datasets and the clients' computational heterogeneity. In particular, the presence of highly non-i.i.d. data severely impairs both the performance of the trained neural network and its convergence rate, increasing the number of communication rounds requested to reach a performance comparable to that of the centralized scenario. As a solution, we propose FedSeq, a novel framework leveraging the sequential training of subgroups of heterogeneous clients, i.e. superclients, to emulate the centralized paradigm in a privacy-compliant way. Given a fixed budget of communication rounds, we show that FedSeq outperforms or match several state-of-the-art federated algorithms in terms of final performance and speed of convergence. Finally, our method can be easily integrated with other approaches available in the literature. Empirical results show that combining existing algorithms with FedSeq further improves its final performance and convergence speed. We test our method on CIFAR-10 and CIFAR-100 and prove its effectiveness in both i.i.d. and non-i.i.d. scenarios.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> tables/conv_rates_sup.tex <==
% \begin{table*}[]
% \centering
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{lllllllllll}
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{Dataset}} &
%       \multirow{2}{*}{Method} &
%       \multicolumn{3}{c}{$\alpha  = 0$} &
%       \multicolumn{3}{c}{$\alpha  = 0.2$} &
%       \multicolumn{3}{c}{$\alpha  = 0.5$} \\
%     \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} &
%       &
%       \multicolumn{1}{c}{75\%} &
%       \multicolumn{1}{c}{85\%} &
%       \multicolumn{1}{c}{95\%} &
%       \multicolumn{1}{c}{75\%} &
%       \multicolumn{1}{c}{85\%} &
%       \multicolumn{1}{c}{95\%} &
%       \multicolumn{1}{c}{75\%} &
%       \multicolumn{1}{c}{85\%} &
%       \multicolumn{1}{c}{95\%} \\
%      \midrule
%     % content
%     \multirow{9}{*}{CIFAR-10} &
%       FedAvg &
%       4897 (1x) &
%       9221 (1x) &
%       - (--) &
%       2866 (1x) &
%       5339 (1x) &
%       - (--) &
%       2386 (1x) &
%       4585 (1x) &
%       - (--) \\
%      &
%       FedProx &
%       4897 (1x) &
%       9221 (1x) &
%       - (--) &
%       2866 (1x) &
%       5338 (1x) &
%       - (--) &
%       2391 (1x) &
%       4584 (1x) &
%       - (--) \\
%      &
%       SCAFFOLD &
%       &
%       &
%       &
%       &
%       &
%       &
%       &
%       &
%       \\
%      &
%       FedDyn &
%       &
%       &
%       &
%       &
%       &
%       &
%       &
%       &
%       \\
%      \cmidrule(lr){2-2} & 
%       FedSeq (confidence KL) &
%       699 (7,01x) &
%       \textbf{1151 (8,01x)} &
%       \textbf{2893 (--)} &
%       499 (5,74x) &
%       907 (5,89x) &
%       2289 (--) &
%       \textbf{395 (6,04x)} &
%       \textbf{743 (6,17x)} &
%       \textbf{1868 (--)} \\
%      &
%       FedSeq (classifierAll) &
%       \textbf{997 (4,91x)} &
%       \textbf{1812 (5,09x)} &
%       \textbf{5190 (--)} &
%       \textbf{487 (5,89x)} &
%       \textbf{862 (6,19x)} &
%       \textbf{2179 (--)} &
%       \textbf{412 (5,79x)} &
%       \textbf{739 (6,2x)} &
%       1904 (--) \\
%      &
%       FedSeq (confidence KL) + FedProx &
%       \textbf{689 (7,11x)} &
%       1151 (8,01x) &
%       2896 (--) &
%       499 (5,74x) &
%       906 (5,89x) &
%       2285 (--) &
%       395 (6,04x) &
%       744 (6,16x) &
%       1923 (--) \\
%      &
%       FedSeq (confidence KL) + SCAFFOLD &
%       \textbf{} &
%       &
%       &
%       \textbf{} &
%       &
%       \textbf{} &
%       &
%       &
%       \\
%      &
%       FedSeqInter (confidence KL) &
%       893 (5,48x) &
%       1518 (6,07x) &
%       3300 (--) &
%       660 (4,34x) &
%       1210 (4,41x) &
%       2915 (--) &
%       533 (4,48x) &
%       975 (4,7x) &
%       2476 (--) \\
%     \midrule
%     \multirow{9}{*}{CIFAR-100} &
%       FedAvg &
%       15163 (1x) &
%       - (--) &
%       \textbf{- (--)} &
%       6712 (1x) &
%       10677 (1x) &
%       - (--) &
%       6224 (1x) &
%       9811 (1x) &
%       \textbf{- (--)} \\
%      &
%       FedProx &
%       15163 (1x) &
%       - (--) &
%       - (--) &
%       6708 (1x) &
%       10685 (1x) &
%       - (--) &
%       6223 (1x) &
%       9767 (1x) &
%       - (--) \\
%      &
%       SCAFFOLD &
%       &
%       &
%       &
%       &
%       &
%       &
%       &
%       &
%       \\
%      &
%       FedDyn &
%       &
%       &
%       &
%       &
%       &
%       &
%       &
%       &
%       \\
%       \cmidrule(lr){2-2} &
%       FedSeq (confidence KL) &
%       3219 (4,71x) &
%       \textbf{6572 (--)} &
%       - (--) &
%       964 (6,96x) &
%       \textbf{1487 (7,18x)} &
%       8420 (--) &
%       \textbf{883 (7,05x)} &
%       \textbf{1341 (7,32x)} &
%       3130 (--) \\
%      &
%       FedSeq (classifierAll) &
%       4118 (3,68x) &
%       10282 (--) &
%       - (--) &
%       965 (6,96x) &
%       1455 (7,34x) &
%       - (--) &
%       885 (7,03x) &
%       1359 (7,22x) &
%       2816 (--) \\
%      &
%       FedSeq (confidence KL) + FedProx &
%       \textbf{3197 (4,74x)} &
%       6664 (--) &
%       - (--) &
%       \textbf{953 (7,04x)} &
%       1506 (7,09x) &
%       \textbf{3143 (--)} &
%       883 (7,05x) &
%       1343 (7,31x) &
%       3115 (--) \\
%      &
%       FedSeq (confidence KL) + SCAFFOLD &
%       &
%       &
%       &
%       &
%       &
%       &
%       &
%       &
%       \\
%      &
%       FedSeqInter (confidence KL) &
%       3186 (4,76x) &
%       4633 (--) &
%       \textbf{9083 (--)} &
%       1225 (5,48x) &
%       1813 (5,89x) &
%       3093 (--) &
%       1088 (5,72x) &
%       1556 (6,31x) &
%       \textbf{2708 (--)}\\
%      \bottomrule \\
%     \end{tabular}
% }
%     \caption{Convergence rates for the best configurations of FedSeq and SOTAs. For each algorithm we report the round in which it reaches respectively the 75\%, 85\% and 95\% of centralized accuracy. Inside curly braces the speedup relative to FedAvg. "--" means that the algorithm did not reach the target accuracy in the given round budget; "(--)" means that FedAvg did not reach the target accuracy (so we cannot calculate the speedup) \ric{troppo prolissa, ma solo per capirci)}\deb{vedere se metterla tutta o solo una parte (il resto nei supplementary)}}
%     \label{tab:rates}
% \end{table*}

\setlength\dashlinedash{0.5pt}
\setlength\dashlinegap{1.5pt}
\setlength\arrayrulewidth{0.3pt}

\begin{table*}[]
\centering
\label{tab:rates}
\resizebox{\linewidth}{!}{
    \begin{tabular}{lllllllllll}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Dataset}} &
      \multirow{2}{*}{Method} &
      \multicolumn{3}{c}{$\alpha  = 0$} &
      \multicolumn{3}{c}{$\alpha  = 0.2$} &
      \multicolumn{3}{c}{$\alpha  = 0.5$} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} &
       &
      \multicolumn{1}{c}{70\%} &
      \multicolumn{1}{c}{80\%} &
      \multicolumn{1}{c}{90\%} &
      \multicolumn{1}{c}{70\%} &
      \multicolumn{1}{c}{80\%} &
      \multicolumn{1}{c}{90\%} &
      \multicolumn{1}{c}{70\%} &
      \multicolumn{1}{c}{80\%} &
      \multicolumn{1}{c}{90\%} \\
     \midrule
     
    % content
    \multirow{10}{*}{CIFAR-10} &
    %SOTAs
    FedAvg                           & 4036 (1x)    & 7649 (1x)    & - (--)    & 2384 (1x)    & 4507 (1x)    & - (--)    & 1945 (1x)    & 3749 (1x)   & 8791 (1x)    \\
    & FedProx                          & 4036 (1x)    & 7649 (1x)    & - (--)    & 2384 (1x)    & 4507 (1x)    & - (--)    & 1946 (1x)    & 3753 (1x)   & 8786 (1x)    \\
    & SCAFFOLD                         & 2229 (1,81x) & 3914 (1,95x) & 8043 (--) & 2554 (0,93x) & 4771 (0,94x) & - (--)    & 1934 (1,01x) & 3761 (1x)   & 8453 (1,04x) \\
    & FedDyn &
      {\textbf{563 (7,17x)}} &
      \textbf{954 (8,02x)} &
      \textbf{2131 (--)} &
      \textbf{450 (5,3x)} &
      \textbf{797 (5,65x)} &
      \textbf{2059 (--)} &
      \textbf{374 (5,2x)} &
      \textbf{634 (5,91x)} &
      \textbf{1648 (5,33x)} \\
  
    %Ours (intra)
    %\cmidrule(lr){2-2} & 
    %\cdashline{2-11} &
    \cmidrule(lr){2-2} &
     FedSeq\textsuperscript{1} &
      594 (6,79x) &
      991 (7,72x) &
      2047 (--) &
      407 (5,86x) &
      746 (6,04x) &
      1682 (--) &
      325 (5,98x) &
      619 (6,06x) &
      1358 (6,47x) \\
    & FedSeq\textsuperscript{2} &
      873 (4,62x) &
      1502 (5,09x) &
      3677 (--) &
      387 (6,16x) &
      720 (6,26x) &
      1543 (--) &
      323 (6,02x) &
      620 (6,05x) &
      1409 (6,24x) \\
    % Integration with SOTAs
    & FedSeq\textsuperscript{1} + FedProx & 594 (6,79x)  & 991 (7,72x)  & 2046 (--) & 407 (5,86x)  & 746 (6,04x)  & 1682 (--) & 325 (5,98x)  & 619 (6,06x) & 1358 (6,47x) \\
    & FedSeq\textsuperscript{1} + FedDyn  & {\ul {\textbf{345 (11,7x)}}} &
  {\ul {\textbf{581 (13,17x)}}} &
  {\ul {\textbf{1341 (--)}}} &
  {\ul {\textbf{253 (9,42x)}}} &
  {\ul {\textbf{447 (10,08x)}}} &
  {\ul {\textbf{1113 (--)}}} &
  {\ul {\textbf{232 (8,38x)}}} &
  {\ul {\textbf{403 (9,3x)}}} &
  {\ul {\textbf{933 (9,42x)}}}\\
     %\cmidrule(lr){2-2} &
     \cmidrule(lr){2-2} &
    % FedSeqInter
     FedSeqInter\textsuperscript{1}           & 762 (5,3x)   & 1305 (5,86x) & 2492 (--) & \textbf{538 (4,43x)}  & 1004 (4,49x) & 2099 (--) & \textbf{433 (4,49x)}  & \textbf{814 (4,61x)} & 1805 (4,87x) \\
    & FedSeqInter\textsuperscript{1} + FedProx &   \textbf{735 (5,49x)} &	\textbf{1264 (6,05x)} &	\textbf{2388 (--)} &	544 (4,38x)	& \textbf{1000 (4,51x)} &	\textbf{2084 (--)} &	436 (4,46x)	& 825 (4,54x) &	\textbf{1747 (5,03x)}\\
    & FedSeqInter\textsuperscript{1} + FedDyn &    &	 &	 &	&  & &	&  &\\
    \midrule 
    \multirow{10}{*}{CIFAR-100} &
    %SOTAs
    FedAvg &
      14412 (1x) &
      - (--) &
      - (--) &
      6409 (1x) &
      10253 (1x) &
      - (--) &
      5879 (1x) &
      9331 (1x) &
      - (--) \\
    & FedProx &
      14412 (1x) &
      - (--) &
      - (--) &
      6363 (1,01x) &
      10277 (1x) &
      - (--) &
      5918 (0,99x) &
      9250 (1,01x) &
      - (--) \\
    & SCAFFOLD &
      14483 (1x) &
      - (--) &
      - (--) &
      7088 (0,9x) &
      10191 (1,01x) &
      17200 (--) &
      6951 (0,85x) &
      10373 (0,9x) &
      16744 (--) \\
    & FedDyn &
      {\ul \textbf{- (--)}} &
      {\ul \textbf{- (--)}} &
      \textbf{- (--)} &
      \textbf{1031 (6,22x)} &
      \textbf{1603 (6,4x)} &
      \textbf{2634 (--)} &
      \textbf{868 (6,77x)} &
      \textbf{1433 (6,51x)} &
      \textbf{3018 (--)} \\
  
    %Ours (intra)
    \cmidrule(lr){2-2} & 
    %\cdashline{2-2} &
    FedSeq\textsuperscript{1} &
      3009 (4,79x) &
      5780 (--) &
      - (--) &
      {\ul \textbf{901 (7,11x)}} &
      1421 (7,22x) &
      \textbf{3436 (--)} &
      854 (6,88x) &
      {\ul \textbf{1264 (7,38x)}} &
      {\ul \textbf{2812 (--)}} \\
    & FedSeq\textsuperscript{2} &
      3968 (3,63x) &
      9378 (--) &
      - (--) &
      {\ul \textbf{922 (6,95x)}} &
      {\ul \textbf{1396 (7,34x)}} &
      {\ul \textbf{3924 (--)}} &
      {\ul \textbf{843 (6,97x)}} &
      1266 (7,37x) &
      {\ul \textbf{2713 (--)}} \\
    % Integration with SOTAs
    & FedSeq\textsuperscript{1} + FedProx &
      2946 (4,89x) &
      6005 (--) &
      - (--) &
      898 (7,14x) &
      1397 (7,34x) &
      3033 (--) &
      843 (6,97x) &
      1298 (7,19x) &
      2833 (--) \\
    & FedSeq\textsuperscript{1} + FedDyn &
       {\ul {\textbf{1914 (7,53x)}}} &
          {\ul {\textbf{3293 (--)}}} &
          {\ul {\textbf{7511 (--)}}} &
          {\ul {\textbf{556 (11,53x)}}} &
          {\ul {\textbf{987 (10,39x)}}} &
          {\ul {\textbf{2014 (--)}}} &
          {\ul {\textbf{541 (10,87x)}}} &
          {\ul {\textbf{957 (9,75x)}}} &
          {\ul {\textbf{1912 (--)}}} \\
     \cmidrule(lr){2-2} &
     %\cdashline{2-2} &
    % FedSeqInter
     FedSeqInter\textsuperscript{1} &
      3028 (4,76x) &
      4333 (--) &
      8494 (--) &
      1177 (5,45x) &
      1734 (5,91x) &
      3004 (--) &
      1034 (5,69x) &
      \textbf{1524 (6,12x)} &
      2675 (--) \\
    & FedSeqInter\textsuperscript{1} + FedProx &
       \textbf{3027 (4,76x)} &	\textbf{4310 (--)} &	\textbf{7149 (--)} &	\textbf{1163 (5,51x)} &	\textbf{1721 (5,96x)} &	\textbf{2915 (--)} &	\textbf{1033 (5,69x)} &	1525 (6,12x) &	\textbf{2616 (--)} \\
     \bottomrule \\
    \end{tabular}
}
    \caption{Convergence rates for the best configurations of FedSeq (1: $\{ \psi_\textnormal{conf}, \phi_\textnormal{greedy}, \tau_{KL}\}$, 2: $\{ \psi_\textnormal{clfAll}, \phi_\textnormal{greedy}, \tau_{cosine}\}$) and SOTAs. We report the round in which the 70\%, 80\% and 90\% of centralized accuracy is reached (\quotes{--} if the target accuracy was not reached), together with the speedup relative to FedAvg (\quotes{--} if FedAvg did not reach the target accuracy).}%\deb{aggiungere risultati mancanti}} %\deb{vedere se metterla tutta o solo una parte (il resto nei supplementary)} \ric{Ricordiamoci di risistemare i grassetti/sottolineati: in generale userei il grassetto per il migliore del gruppo (es. SOTA, nostro intra, nostro inter, nostro+SOTA, nostro inter+SOTA) e il sottolineato per il migliore globale, per colonna}}
\end{table*}
